S-Store: Streaming Meets Transaction Processing

Stream processing addresses the needs of real-time applications. Transaction processing addresses the coordination and safety of short atomic computations. Heretofore, these two modes of operation existed in separate, stove-piped systems. In this work, we attempt to fuse the two computational paradigms in a single system called S-Store. In this way, S-Store can simultaneously accommodate OLTP and streaming applications. We present a simple transaction model for streams that integrates seamlessly with a traditional OLTP system. We chose to build S-Store as an extension of H-Store, an open-source, in-memory, distributed OLTP database system. By implementing S-Store in this way, we can make use of the transaction processing facilities that H-Store already supports, and we can concentrate on the additional implementation features that are needed to support streaming. Similar implementations could be done using other main-memory OLTP platforms. We show that we can actually achieve higher throughput for streaming workloads in S-Store than an equivalent deployment in H-Store alone. We also show how this can be achieved within H-Store with the addition of a modest amount of new functionality. Furthermore, we compare S-Store to two state-of-the-art streaming systems, Spark Streaming and Storm, and show how S-Store matches and sometimes exceeds their performance while providing stronger transactional guarantees.

==> definitions.tex <==
\section{Definitions and Assumptions} \label{sec:definitions}

\begin{definition}
{\bf Database} is a collection of relations, streams, and windows.
\end{definition}

\begin{definition}
{\bf Relation} is an unordered, bounded collection of tuples. 
\end{definition}

\begin{definition}
{\bf Stream} is an ordered, unbounded collection of tuples. 
\end{definition}

\begin{definition}
{\bf Atomic Batch} is a finite, contiguous subsequence of a stream that must be processed atomically as an indivisible unit. Atomic batches do not overlap.
\end{definition}

\begin{definition}
{\bf Window} is a finite, contiguous subsequence of a stream.
\end{definition}

\begin{definition}
{\bf Sliding Window} is a window which has a fixed size and a fixed slide; slide $\leq$ size and specifies the distance between two consecutive windows.
\end{definition}

\begin{definition}
{\bf Time-based Sliding Window} is a sliding window for which size and slide are defined in terms of tuple timestamps.
\end{definition}

\begin{definition}
{\bf Tuple-based Sliding Window} is a sliding window for which size and slide are defined in terms of the number of tuples.
\end{definition}

\begin{definition}
{\bf Transaction} represents a finite unit of work (i.e., a finite sequence of read and write operations) performed over a given database. Each transaction has a definition and possibly many executions (i.e., instances).
\end{definition}

\begin{definition}
{\bf OLTP Transaction} is a transaction that involves operations only over relations.
\end{definition}

\begin{definition}
{\bf Streaming Transaction} is a transaction that involves operations over one or more streams (i.e., it can additionally involve operations over windows and/or relations).
\end{definition}

\begin{definition}
{\bf Workflow} is a directed acyclic graph (DAG) in which nodes represent streaming transactions and edges represent an execution ordering between them.
\end{definition}

\begin{definition}
{\bf Nested Transaction} is a group of transactions with a partial order defined among them. A nested transaction will commit if and only if all of its transactions commit, and will abort if one or more of its transactions abort.
\end{definition}

\begin{definition}
{\bf Trigger}, defined over a stream (or over a sliding window), specifies a finite computation that must be automatically executed in response to append of a new atomic batch to that stream (or append of at least a slide worth of tuples to that window signaling the availability of a new full window).
\end{definition}

\subsection{Assumptions}

\begin{itemize}

\item Stream order 

\item Single computational node, multiple processing sites per node.

\item Serial transaction execution per site.

\item Transactions are defined as stored procedures with input parameters.

\end{itemize}


==> formal.tex <==
% Formal stuff for isolation

Consider a workflow $W$ of $n$ streaming transactions $T_i$, $1 \leq i \leq n$. $W$ is a directed acyclic graph $G=(V,E)$, where $V=\{T_1, \ldots, T_n\}$ and $E \subseteq V \times V$, where $(T_i, T_j) \in E$ means that $T_i$ must precede $T_j$.

Being a DAG, $G$ has at least one topological ordering. A topological ordering of $G$ is an ordering of its nodes $T_i \in V$ such that for every edge $(T_i, T_j) \in E$ we have $i < j$. Each topological ordering of $G$ is essentially some permutation of $V$.

Without loss of generality:
(i) Let us focus on one specific topological ordering of $G$ and call it $O$;
(ii) For ease of notation, let us simply assume that $O$ corresponds to the identity permutation such that it represents: $T_1 < T_2 < .. < T_n$.

$T_i$ represents a transaction definition $T_i(s_i, w_i, p_i)$, where
$s_i$ denotes all private stream inputs of $T_i$,
$w_i$ denotes all private window inputs of $T_i$,
$p_i$ denotes all public table partition inputs of $T_i$.

$T_i^j$ represents the $j^{\text{th}}$ transaction execution of $T_i$, $T_i^j(s_i.b_j, w_i, p_i)$, where $b_j$ denotes the  $j^{\text{th}}$ atomic batch of $s_i$.

A workflow $W$ is executed in rounds of atomic batches $1 \leq r < \infty$, such that:

For round $r=1$, atomic batch 1 from all streaming inputs into $W$ generates a sequence of TE's $T_i^1(s_i.b_1, w_i, p_i)$ for each $T_i$.
 
For round $r=2$, atomic batch 2 from all streaming inputs into $W$ generates a sequence of TE's $T_i^2(s_i.b_2, w_i, p_i)$ for each $T_i$. 

$\ldots$, and so on.

Note that this execution generates an unbounded schedule. However, as of a specific round $r=R$, we generate a bounded schedule that consists of $R*n$ TE's: $1 \leq r \leq R, 1 \leq i \leq n, T_i^r(s_i.b_r, w_i, p_i)$.

In the traditional ACID model of databases, any permutation of these $R*n$ TE's is considered to be a valid/correct, serial schedule.

In our model, we additionally have:

\begin{enumerate}

\item {\em Workflow order constraints:}
Consider the topological ordering $O$ of $W$ as defined above. Then for any given round $r$, it must hold that:

$T_1^r(s_1.b_r, w_1, p_1) < T_2^r(s_2.b_r, w_2, p_2) < \ldots < T_n^r(s_n.b_r, w_i, p_i)$ 

\item {\em Stream order constraints:}
For any given transaction $T_i$, as of any round $r=R$, the following must hold:

$T_i^1(s_i.b_1, w_i, p_i) < T_i^2(s_i.b_2, w_i, p_i) < \ldots < T_i^R(s_i.b_R, w_i, p_i)$

\end{enumerate}

Any bounded schedule of $W$ that meets the above two ordering constraints is a correct schedule.

{\bf OLTP Transactions:} Any OLTP transaction execution $T_i^j(p_i)$ can interleave anywhere in a correct bounded schedule of $W$. The resulting bounded schedule would still be correct.

{\bf Nested Transactions:} Any streaming transaction $T_i$ in workflow $W$ can be defined as a nested transaction that consists of children $T_{i1}, \ldots, T_{im}$. In this case, $T_{i1}, \ldots, T_{im}$ must obey the partial order defined for $T_i$ for every execution round $r$, $1 \leq r < \infty$. This means that no other streaming or OLTP transaction instance can interleave with $T_{i1}, \ldots, T_{im}$ for any given execution round.


==> hstore.tex <==
\section{H-Store Overview} \label{sec:hstore}

We build the XXX prototype on top of H-Store - an open-source, main-memory OLTP engine that was developed at Brown and MIT \cite{hstore} and formed the basis for the design of the VoltDB NewSQL database system \cite{voltdb}. This section will briefly describe the architecture and implementation of H-Store.

All transactions in H-Store must be predefined as stored procedures with input parameters. A {\em stored procedure} (SP) is a transaction definition that specifies the code for a transaction execution. The stored procedure code is a mixture of SQL and Java. A {\em transaction execution} (TE) is an instantiation of a transaction definition. It is what you get when you bind input parameters to real values and run the transaction. In general, a given stored procedure will, over time,  generate many transaction executions. Transaction executions are submitted to H-Store, and the H-Store scheduler executes them in whatever order it deems best. 

H-Store follows a typical distributed architecture in which there is a layer (called {\em the partion engine (PE)}) that is responsible for managing transaction distribution, scheduling, coordination, and recovery. The PE itself is built on top of another layer that is responsible for the local execution of SQL queries (called {\em the execution engine (EE)}). In the case of H-Store, the PE is written in Java and the EE is written in C++ (for easier control and tuning of the underlying system resources). A client program connects to the PE via a stored procedure execution request. If the stored procedure requires SQL processing, then the EE is invoked with these sub-requests.

An H-Store database is partitioned across multiple sites \cite{pavlo12}. A transaction is executed on the sites that hold the data that it needs. If the data is partitioned carefully, most transactions will only need data from a single site. Single-sited transactions are run serially on that node, thereby eliminating the need for fine-grained locks and latches.

H-Store provides recovery through a checkpointing and command-logging mechanism \cite{malviya14}. Periodically, the system creates a persistent snapshot or checkpoint of the current committed state of the database. To create a snapshot, the system must quiesce its running transactions. That is, it must delay new transactions and wait until all in-flight transactions commit or abort. When the system has quiesced, it persistently records the state of {\em all} tables. Thus, the snapshot captures a complete and consistent state of the database.

After a snapshot is complete, the system resumes normal operation. Every time it commits a transaction, it writes a command-log record containing the name of the corresponding stored procedure along with its input parameters. This command-log record must be made persistent before its transaction can commit. In order to minimize intereactions with the slow persistent store, H-Store offers a group-commit mechanism. Group-commit collects a batch of commit records and writes them as a group to persistent storage. This amortizes the I/O cost at the expense of delaying actual commits.

Note that updates can be done in-place, since a recovery action forces the system back to the last checkpoint, thereby, wiping out all changes that have been made since then. Thus, an undo log is unnecessary.

On recovery, the system's state is restored to the latest snapshot, and the command-log is replayed. That is, each command-log record allows the system to re-execute its associated stored procedure with the same arguments that it did before the failure.

It should be noted that replaying the command-log can require more work than using an Aries-style physical write-ahead log (WAL). H-Store is willing to accept this fact, since failure is relatively rare, and command-logging is lighter-weight than WAL during normal operation \cite{malviya14}.
55

==> version0/architecture.tex <==
\section{Architectural Overview} \label{s:architecture}

\todo[inline]{
We may want to detail the H-Store description if needed.
}

S-Store extends the architecture of H-Store \cite{hstore}. In a nutshell,
H-Store is a high-performance, in-memory, distributed OLTP system designed
for shared-nothing clusters. It targets OLTP workloads with short-lived
transactions, which are pre-defined as parametric stored procedures
(i.e., SQL queries embedded in Java programs) that get instantiated by client
requests at run time. Data is carefully partitioned and transactions that
can be executed on a single partition are run serially on that partition,
eliminating the need for locks and latches. H-Store's database designer
strives to minimize the number of distributed transactions to reduce the
overhead of coordination across the partitions \cite{pavlo12}.
Fault tolerance is achieved based on a technique that combines command logging
and periodic snapshots \cite{malviya14}.

S-Store builds on H-Store’s architecture, reusing its core data management
primitives such as tables and stored procedures. In addition, it introduces
a number of new primitives for supporting stream processing natively.
S-Store’s key extensions include:

\compactlist

\item {\bf New constructs for streams, windows, triggers, and workflows:}
Streams differentiate continuously streaming state from regular stored state;
windows define finite chunks of state over (possibly unbounded) streams;
triggers are used to indicate computations to be invoked for newly generated
data; and workflows refer to pipelines of dependent transactions triggered
by common streaming input(s).

\item {\bf Stream-oriented transaction model:}
We define a streaming transaction in S-Store as a stored procedure with a
streaming input that is invoked by newly arriving stream tuple(s) on that
input.
%Thus, streaming transactions are data-driven, whereas regular OLTP
%transactions are operation-driven.

\item {\bf Uniform state management:}
H-Store’s in-memory tables are used for representing all states including
streams and windows, making state access both efficient and
transactionally safe. Furthermore, S-Store provides automatic garbage
collection mechanisms for tuples that expire from stream or window state.

\item {\bf Data-driven processing via triggers:}
Special insert triggers are defined on stream or window state in order to
enable push-based, data-driven processing in S-Store. There are two types of
triggers: engine triggers at the query level (SQL) and front-end triggers
at the stored procedure level (Java). The former enable continuous processing
for a given transaction, while the latter enable composing workflows of
transactions.

\compactend

\missingfigure[figwidth=\columnwidth]{
Need an architecture figure with all important components,
showing the ones added by S-Store.
}

As shown in Figure \ref{f:3layers},
S-Store follows H-Store's three-layer transaction execution stack
that consists of the client application, the partition engine,
and the execution engine. The native stream processing extensions described
above help S-Store use this stack in the most efficient way by embedding
the required functionality in the proper engine layers, thereby avoiding
redundant computations, communication across the layers, and the need to
poll for new data.
\todo[inline]{Detail the comparison.}

\begin{figure*}[t]
\begin{center}
\subfigure[H-Store]{
    \includegraphics[width=0.45\textwidth]{3layers-hstore.png}
    \label{f:3layers-hstore}
}
\subfigure[H-Store]{
    \includegraphics[width=0.48\textwidth]{3layers-sstore.png}
    \label{f:3layers-sstore}
}
\caption{Three Layers of Transaction Execution}
\label{f:3layers}
\end{center}
\end{figure*}

Figure \ref{f:voterwinsstore} shows how our running example would be
implemented with S-Store.
\todo[inline]{Describe the figure.}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{voterwinsstore.png}
\caption{Streaming Voter with S-Store}
\label{f:voterwinsstore}
\end{figure}

Although discussed within the context of the H-Store OLTP engine in this paper,
we believe that the architectural additions described above generally apply
when extending any in-memory OLTP engine with streams.
The two-layer engine is the only H-Store-specific part of our design,
which essentially leads to having two levels of triggers in the engine.
We believe that all of our extensions are conceptually needed in any OLTP
engine and trigger is the key construct for data-driven processing
and to avoid the need for polling and redundant communication,
even in a single-layer engine.
\todo[inline]{Incorporate Andy's input:}
- Main reasons for the two-layered design: It's easier for customers to write
stored procedures in Java, while it's better to keep all of the storage +
memory management in C++ and avoid the GC.

- PE: Anything dealing with the network, query planning, scheduling,
txn management, stored procedures.

- EE: Low-level query operator execution, storage, indexes.

- H-Store vs. other main-memory OLTP:
The coarse-grained partition locks, single-threaded execution engines,
logical logging, and being optimized only for stored procedures.

==> version0/challenges.tex <==
\section{Research Challenges} \label{s:challenges}

\todo[inline]{
This part needs to be rewritten.
}

Building an integrated system for stream and transaction system such as
S-Store raises a number of interesting research challenges. Following is
a list of problems that are in our current research agenda:

\compactlist

\item Workload partitioning:
S-Store takes its foundation from a distributed main-memory OLTP system
that achieves high transactional performance by carefully partitioning
its data and transaction workload onto a cluster of nodes, each of which
itself is running one or more partition engine instances with its own
shard of data. This is achieved using an automatic designer that decides on
the data partitions in a way to minimize the number of distributed
transactions required for a given type of workload.
In the presence of streaming inputs and complex workflows of transactions
that execute in a push-based manner, the designer needs to additionally
decide how to partition these streaming inputs as well as
where to run different transactions that comprise a given workflow.
We have been working on a new cost model to guide the designer in making
these decisions given the new forms of parallelism opportunities
and data dependency constraints in S-Store workloads.

\item Transaction management:
Our research in this area is focusing on two key questions:
when do we need transactional semantics for streams and how
do we define a transaction when streaming data is involved?
S-Store currently follows a basic stream-oriented transaction model
that uses newly arriving tuples to trigger transaction requests and
to determine transactional boundaries on continuous data. We have been
working on generalizing this model in a way to support a variety of
application semantics in a flexible and performant way.

\item Handling mixed and dynamic workloads:
S-Store can potentially support mixed workloads with regular OLTP
transactions, streaming OLTP transactions, as well as adhoc transactions.
Furthermore, workload conditions can change over time.
It is an interesting question how to prioritize the scheduling of such
mixed and complex workloads as well as support more elastic workload
partitioning under dynamic settings.

\item Performance analysis and hardware optimization:
Like H-Store, S-Store has great potential to optimize its transactional
performance further by leveraging modern hardware architectures
(e.g., multiple cores, non-volatile memory). Our future work includes
performing a rigorous software performance analysis of S-Store in
a way to identify bottlenecks and fix them exploiting modern hardware.

\compactend

==> version0/conclusions.tex <==
\section{Conclusions} \label{s:conclusions}

==> version0/experiments.tex <==
\section{Experiments} \label{s:experiments}

\subsection{Goals and Setup}

\subsection{Streaming TPC-E}

- goals: to show that we can support complex/realistic benchmarks;
to show performance benefits over H-Store.

- describe Streaming TPC-E.

- describe H-Store and S-Store implementations.

- results with H-Store and S-Store.

\subsection{Streaming Voter}

- goals: to show performance benefits over H-store on a simpler benchmark
(paper's running example);
to compare against Spark-Streaming and Twitter-Storm
(with different transactional guarantees).

- describe Spark-Streaming and Twitter-Storm implementations.

- results with H-Store, S-Store, Spark-Streaming (exactly once),
Twitter-Storm (at least once), Twitter-Storm+Trident (exactly once)

- if feasible, results with Spark and Twitter giving equivalent guarantees
as S-Store.

\subsection{Streaming WordCount}

- goals: to compare against Spark-Streaming and Twitter-Storm on one of their
own benchmarks; both on single and multiple partitions.

- describe Streaming WordCount.

- describe implementations on S-Store, Spark, Storm.

- results (single-node + multi-node).

\subsection{Discussion}

\begin{comment}

\section{Preliminary Results} \label{s:experiments}

\begin{figure}
\centering
\includegraphics[width=3.0in]{svoter2}
\caption{Streaming Voter Benchmark}
\label{f:svoter2}
\end{figure}

We have compared S-Store's transaction throughput performance against
H-Store's on a streaming version of the Voter Benchmark \cite{benchmarks}.
This benchmark originally models a leader-board application where
a number of contestants participate in a talent show and users call in to
vote on their favorite contestants. Each phone call invokes a new transaction
that updates the total number of votes for each contestant after a number of
validity checks according to the voting rules. Valid votes must be permanently
recorded in the system as well as updating a number of statistical views
over these (e.g., total number of votes per contestant, per state,
and per voting phone number; top-k contestants, etc.).
We have added two streaming extensions to this benchmark:
a stream of votes as input and a sliding window aggregate computation.
We have then implemented this streaming version with S-Store as well as
with H-Store. The S-Store implementation uses the new stream processing
constructs embedded into the execution engine layer such as streams,
windows, engine triggers, whereas the H-Store implementation simulates the
same functionality using the available constructs of H-Store.
Figure \ref{f:svoter2} shows how each of these variants perform for a
tuple-based window of size 100 as the window slide varies
between 1 and 100 (tumbling window). In all of these experiments, S-Store
outperforms H-Store by a factor of about 50\%. The performance gap slightly
decreases as slide increases, since in this case, H-Store has to make
fewer additional computations and calls to the execution engine for
simulating the equivalent windowing behavior.

We are currently extending our experimental study to benchmark S-Store
against H-Store and other alternative stream processing system (e.g.,
\cite{storm}, \cite{zaharia13-short}) using more complex benchmarks
such as a streaming version of the TCP-E OLTP benchmark \cite{tpc-e}.

\end{comment}

==> version0/implementation.tex <==
\section{Implementation} \label{s:implementation}

==> version0/introduction.tex <==
\section{Introduction} \label{s:introduction}

Managing high-speed data streams generated in real time is an integral part of
today’s big data applications. In a wide range of domains from social media to 
financial trading, there is a growing need to seamlessly support incremental
processing as new data is generated. At the same time, the system must ingest
some or all of this data into a persistent store for on-demand transaction or
analytical processing. In particular, for applications with high-velocity data
updating a large persistent state, there is need to manage streaming and
non-streaming state side by side, in a way to ensure transactional integrity
and performance. Examples include leader-board maintenance, multi-player
online games, real-time financial trading, and online advertising.

It has been more than a decade since the first stream processing engines
were built. As these research prototypes moved into the commercial world,
the customer applications that they were used for were rarely pure stream
processing. They often required storage as a way to record the past for
comparison with the present. Thus, the obvious solution was to bolt on a
DBMS, but the solutions were very unsatisfying because they ignored the
need for consistency between streaming results and stored state.

Today’s stream processing systems (stream databases, CEP engines,
distributed real-time computation frameworks such as \cite{streambase},
\cite{oracle-cep}, \cite{storm}) still lack the required transactional
robustness, while OLTP databases do not provide native support for
data-driven processing. In this work, our goal is to fill this gap by
building a single system that can scale to support stream and transaction
processing under the same hood. We believe that modern distributed main-memory
OLTP platforms such as H-Store \cite{hstore} provide a suitable
foundation for building such a system, since: first, they are more
light-weight than their traditional disk-based counterparts; second, like 
streaming engines, they offer lower latency via in-memory processing;
and last but
not least, they provide strong support for state and transaction management.
Thus, we introduce S-Store, a streaming OLTP system that realizes our goal
by extending H-Store with streams.

\subsection{Running Example}

\todo[inline]{
Describe the voter example.
}

\subsection{Contributions}

\todo[inline]{
Summarize contributions and outline of the paper.
}

==> version0/related.tex <==
\section{Related Work} \label{s:related}

Botan et al. have proposed to extend the traditional model to include 
streaming data and continuous queries based on a unified transaction
model \cite{botan-edbt12}... logical model, tested on a stream
processing system, stream-oriented transactions, but no nested transactions...

Zaharia et al.'s batch-based model and exactly-once consistency guarantee
\cite{zaharia13}...

Google MillWheel \cite{millwheel}...

Twitter Storm/Trident, at-least-once or exactly-once, different programming
model \cite{storm}...

==> version0/transactions.tex <==
\section{S-Store Transaction Model} \label{s:transactions}

\subsection{Overview}

In S-Store, all {\em state} is kept in in-memory tables like in H-Store.
In addition to regular tables, one can also define tables to represent
stream state and window state.

S-Store supports regular {\em OLTP transactions} (that only involve access to
regular tables) as well as {\em streaming transactions} (that involve access to
streams or windows along with regular tables).
OLTP transactions are pre-defined as parametric stored procedures
(i.e., SQL queries embedded in Java programs) that get instantiated
by client requests at run time.
Streaming transactions are defined in the same manner except that they get
instantiated by newly arriving data on streaming inputs rather than by client
transaction requests. In other words, streaming transactions are
{\em data-driven} while OLTP transactions are operation-driven.
Furthermore, S-Store allows multiple streaming transactions to be composed
into a {\em transactional workflow}.

\subsection{Streaming Transactions}

A stored procedure that defines a streaming transaction involves a sequence of
SQL commands that get triggered by new tuple insertions into stream or window
state. Each new ``batch" of tuples inserted into the input stream of this
stored procedure instantiates a new transaction that executes this sequence.
A {\em batch} is a sequence of stream tuples that logically belong together
to be processed as an atomic unit and can be defined in an application-specific
way. For example, tuples with a common timestamp might be specified as a batch,
or tuples that include sales orders from a common business transaction might be
specified as a batch.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{txn-example.png}
\caption{Streaming transaction example}
\label{f:txn-example}
\end{figure}

The streaming transaction shown in Figure \ref{f:txn-example} selects
tuples with values above 10 from a stream, constructs a window out
of them (assume a window defined as a tuple-based tumbling window of size 2),
computes an average of the values in each window, and then the results are
written to a table. More specifically, input batch (a,b) initiates a
transaction instance T1, where:

\begin{enumerate}[(i)]

\setlength{\itemsep}{0pt}
\setlength{\parsep}{3pt}
\setlength{\topsep}{3pt}
\setlength{\partopsep}{0pt}
\setlength{\leftmargin}{1.5em}
\setlength{\labelwidth}{1em}
\setlength{\labelsep}{0.5em}

\item the first SQL statement writes (a,b) into stream S,

\item insert trigger defined on S fires the second SQL statement that selects
tuples with values above 10 (say, (a) qualifies) and writes them into stream
S',

\item insert trigger defined on S' fires the third SQL statement writing
(a) into window W,

\item window insert trigger defined on W fires the last SQL statement if there
is a full window, which then computes an average for that window and writes
the result into table T.

\end{enumerate}

T1 {\em commits} when there are no more SQL statements or triggers to execute.
Then the system can initiate the next transaction instance T2 for the next
input batch (c,d,e), and so on. This entails that subsequent instances of a
streaming transaction executed on a given node are inherently serial.

Note that while each transaction instance is executed {\em atomically} with
respect to the input batches that triggers it, not all SQL statements are
necessarily executed in every instance. For example, T1 will only execute up
to step (iv) since there is no full window to trigger the last statement yet.
A similar situation could arise if none of the tuples in a given batch
qualified the filter predicate in step (ii), committing the transaction
instance right after (ii).

Stream state is garbage collected after all relevant triggers are executed.
So is window state. While no stream state is left behind after a transaction
instance commits, this is not necessarily the case for window state.
For example, T1 will insert (a) into W, but the window insert trigger on W
will not yet fire, i.e., (a) has to be kept in window state W. This means
that state from a transaction instance (T1) can carry over to the subsequent
ones (T2). Furthermore, for correct execution of the streaming transaction,
such state must be protected from {\em side effects} of other transactions.
For example, another OLTP or streaming transaction should not be able to see
or modify any state kept in W between subsequent instantiations of the
streaming transaction (i.e., after T1 commits and before T2 starts).
Such a restriction is not needed for regular table state, e.g., another OLTP
transaction can read/modify table T without causing any side effects on our
streaming transaction's instances.

To protect state that carries over across subsequent instances of a streaming
transaction, we use a {\em nested transaction model}. All such instances are
treated as if they were subtransactions of a common transaction. Any state
that should only be visible to them must be explicitly specified
(W in our example). All other state is treated in the usual way.

Note that subtransactions execute in a serial fashion on a given node and
their order of execution is determined by the input batches, i.e., no
{\em concurrency issues} arise among these subtransactions. On the other hand,
an interesting concurrency scenario might arise within a given subtransaction,
if there were multiple triggers defined on a common stream or window state,
firing at the same time and leading to multiple SQL statements downstream
that might have conflicting access to shared state. In S-Store, we process
the triggers of a transaction instance in a pre-defined order (depth-first)
and therefore this scenario never occurs.

Streaming transactions offer interesting opportunities for
{\em speculative execution}. For example, the batch-based definition of a
streaming transaction leads to the question whether a transaction instance
should be scheduled for execution as soon as the first element of a new
batch arrives (a) or after the whole batch has arrived (a,b).
The first approach may block the execution engine if the input is slow and
the rest of the batch does not arrive right away for the transaction instance
to commit (long-running transaction). On the other hand, the second approach
does not allow making progress with the new tuples as soon as they arrive.
If there is no regular table state (externally visible) involved in a
streaming transaction, then we can safely take the first approach and
execute the transaction instance exploiting the fact that all state is
anyway protected in this case due to our nested transaction model.
On the other hand, if regular table state is involved, we can also
speculatively execute up until the step that involves access to the
table state. In this case, we would only complete the rest of the
execution after we have received the whole batch. In the meantime,
other transactions would be allowed to access the table state.
We currently implement the second approach in S-Store and plan to
investigate speculative transaction execution opportunities
as part of our future work.

\subsection{Workflows of Streaming Transactions}

In S-Store, multiple streaming transactions can be composed into a
transactional workflow. In this case, additional data dependency scenarios
arise across instances of different transactions that are part of the same
workflow (in addition to the ones across instances of the same transaction
as we have discussed in the previous section). We can capture them using
another level of transaction nesting in our model.

\begin{figure}[t]
\centering
\includegraphics[width=0.5\columnwidth]{workflow-example.png}
\caption{Streaming workflow example}
\label{f:workflow-example}
\end{figure}

For example,
the workflow in Figure \ref{f:workflow-example} consists of three streaming
transactions X, Y, and Z. $S_{xy}$ represents the stream that flows from
X to Y, and $S_{yz}$ represents the stream that flows from Y to Z.
Furthermore, X and Y both access a common regular table T.
We consider X, Y, and Z to be subtransactions of a common transaction for the
whole workflow. This way we can protect states $S_{xy}$ and $S_{yz}$ from the
access of all OLTP and streaming transactions that are external to this
workflow.
Assume that the whole workflow runs on the same node, i.e., instances
of X, Y, and Z do not execute in parallel. While instances of each transaction
execute serially among themselves ($X1 \rightarrow X2 \rightarrow X3;
Y1 \rightarrow Y2 \rightarrow Y3; Z1 \rightarrow Z2 \rightarrow Z3$),
they can interleave in multiple different ways (though not completely
arbitrarily) across instances of different transactions.
For example, the following would both be possible orderings:

(i) $X1 \rightarrow Y1 \rightarrow Z1 \rightarrow X2 \rightarrow Y2 \rightarrow
Z2 \rightarrow X3 \rightarrow Y3 \rightarrow Z3$

(ii) $X1 \rightarrow X2 \rightarrow Y1 \rightarrow X3 \rightarrow Z1
\rightarrow Y2 \rightarrow Y3 \rightarrow Z2 \rightarrow Z3$

The question is whether all orderings are ``serializable" with respect to
the data dependencies within the workflow. If there is no shared non-streaming
state like T, this would certainly be the case. Otherwise, depending on the
nature of how T is shared across X and Y, we may want to disallow orderings
like in (ii), since it may be that effects of processing batch (a,b)
through X1 must be seen by Y1 first, before X2 overwrites them
by processing batch (c,d,e)...
